Spectral Evolution of Ultraluminous X-ray Pulsar NGC 300 ULX-1

We report on results from a one-year soft X-ray observing campaign of the ultraluminous X-ray pulsar NGC 300 ULX-1 by the Neutron star Interior Composition Explorer (NICER) during 2018--2019. Our analysis also made use of data from Swift/XRT and XMM-Newton in order to model and remove contamination from the nearby eclipsing X-ray binary NGC 300 X-1. We constructed and fitted a series of 5-day averaged NICER spectra of NGC 300 ULX-1 in the 0.4--4.0 keV range to evaluate the long-term spectral evolution of the source, and found that an absorbed power-law model provided the best fit overall. Over the course of our observations, the source flux (0.4--4.0 keV; absorbed) dimmed from $2\times10^{-12}$ to below $10^{-13}{\rm\,erg\,s^{-1}\,cm^{-2}}$ and the spectrum softened, with the photon index going from $\Gamma\approx1.6$ to $\Gamma\approx2.6$. We interpret the spectral softening as reprocessed emission from the accretion disk edge coming into view while the pulsar was obscured by the possibly precessing disk. Some spectral fits were significantly improved by the inclusion of a disk blackbody component, and we surmise that this could be due to the pulsar emerging in between obscuration episodes by partial covering absorbers. We posit that we observed a low-flux state of the system (due to line-of-sight absorption) punctuated by the occasional appearance of the pulsar, indicating short-term source variability nested in longer-term accretion disk precession timescales.

==> tikz.tex <==
\begin{figure*}
    \centering
\begin{tikzpicture}[
    node distance = 0mm,
TN/.style args = {#1/#2}{% as Transparency Node
    fill=#1,
    fill opacity=#2,
    text opacity=1, align=flush left,
    inner sep=1mm, outer sep=0.25mm, below},
   TN/.default = gray!50/0.5,
      L/.style = {% as Line
    draw=gray, line width=1mm,
    {Bar[width=4mm,line width=0.4pt]}-{Bar[width=4mm,line width=0.4pt]}
                 }
                    ]
\draw[L]    ( 0,0)  coordinate (s)
                    node[above=2mm] {2017/04/15} -- + 
            (17.5,0)  node[above=2mm] {2019/05/02};
\draw (3.1,0) -- + (0,-2.4)
        node (e1)   [TN]              {1881}
        node (e1a)  [TN,below=of e1]  {born in the Austrian part\\
                                       of the Austria-Hungarian\\
                                       Empire};
\draw (3.5,0) -- + (0,-0.4) 
        node (e2)   [TN=blue!30/0.3]  {1885}
        node (e2a)  [TN=blue!30/0.7,
                     below=of e2]    {Publication of Darwin's\\
                                      Evolutionary Theory};
\end{tikzpicture}
\end{figure*}

